Adaptive Bayesian Beamforming for Imaging by Marginalizing the Speed of Sound

Imaging methods based on array signal processing often require a fixed propagation speed of the medium, or speed of sound (SoS) for methods based on acoustic signals. The resolution of the images formed using these methods is strongly affected by the assumed SoS, which, due to multipath, nonlinear propagation, and non-uniform mediums, is challenging at best to select. In this letter, we propose a Bayesian approach to marginalize the influence of the SoS on beamformers for imaging. We adapt Bayesian direction-of-arrival estimation to an imaging setting and integrate a popular minimum variance beamformer over the posterior of the SoS. To solve the Bayesian integral efficiently, we use numerical Gauss quadrature. We apply our beamforming approach to shallow water sonar imaging where multipath and nonlinear propagation is abundant. We compare against the minimum variance distortionless response (MVDR) beamformer and demonstrate that its Bayesian counterpart achieves improved range and azimuthal resolution while effectively suppressing multipath artifacts.

==> plots/bayes_8_azim_resol.tex <==
\addplot[very thick,color=color3] coordinates {
(-5.0, 8.107668580691056e-5)
(-4.96078431372549, 8.438662979887097e-5)
(-4.921568627450981, 6.362625978267433e-5)
(-4.88235294117647, 4.3744760586660466e-5)
(-4.8431372549019605, 3.5550194455775826e-5)
(-4.803921568627451, 3.8626198730640436e-5)
(-4.764705882352941, 4.685471579442296e-5)
(-4.7254901960784315, 6.951894561142995e-5)
(-4.686274509803922, 6.364461844454743e-5)
(-4.647058823529412, 4.460234083446399e-5)
(-4.607843137254902, 6.810755677295228e-5)
(-4.568627450980392, 7.792927422179026e-5)
(-4.529411764705882, 9.356720475034174e-5)
(-4.490196078431373, 8.293891301679926e-5)
(-4.450980392156863, 0.00011085065590894952)
(-4.411764705882353, 7.512260593745885e-5)
(-4.372549019607843, 7.419568434980213e-5)
(-4.333333333333333, 6.038367621750369e-5)
(-4.294117647058823, 8.022327722123498e-5)
(-4.254901960784314, 0.00012066370315873604)
(-4.215686274509804, 0.0001218792841043229)
(-4.176470588235294, 0.00010212900232199904)
(-4.137254901960784, 8.544995469862697e-5)
(-4.098039215686274, 8.86767205851419e-5)
(-4.0588235294117645, 9.332689903065046e-5)
(-4.019607843137255, 7.699459838585144e-5)
(-3.980392156862745, 6.220672372267277e-5)
(-3.941176470588235, 5.095647390498278e-5)
(-3.9019607843137254, 3.8006332111656435e-5)
(-3.8627450980392157, 4.9133695532449315e-5)
(-3.8235294117647056, 6.203877538152975e-5)
(-3.784313725490196, 7.533671350957641e-5)
(-3.7450980392156863, 8.212710811219164e-5)
(-3.7058823529411766, 8.665521963854275e-5)
(-3.6666666666666665, 9.745834935481178e-5)
(-3.627450980392157, 0.00011056490950831753)
(-3.588235294117647, 0.00011154650912942793)
(-3.549019607843137, 9.849914876290379e-5)
(-3.5098039215686274, 7.989343505713728e-5)
(-3.4705882352941178, 7.682714125867627e-5)
(-3.4313725490196076, 9.76216121371903e-5)
(-3.392156862745098, 0.0001136121483157945)
(-3.3529411764705883, 0.0001395151424671602)
(-3.313725490196078, 0.00016617402626857558)
(-3.2745098039215685, 0.00017391192249466161)
(-3.235294117647059, 0.0001729499553381248)
(-3.1960784313725488, 0.00015277724306008778)
(-3.156862745098039, 0.00012758606255662135)
(-3.1176470588235294, 0.00011779949215368742)
(-3.0784313725490198, 0.00013696953745138295)
(-3.0392156862745097, 0.00016920901597493218)
(-3.0, 0.00017358225484584073)
(-2.9607843137254903, 0.00016022433364105344)
(-2.9215686274509802, 0.00016981522057333098)
(-2.8823529411764706, 0.00016783600461279987)
(-2.843137254901961, 0.0001809021832877266)
(-2.803921568627451, 0.00020975014341983455)
(-2.764705882352941, 0.00020711787036689947)
(-2.7254901960784315, 0.00015007344936149)
(-2.6862745098039214, 6.2055917024634e-5)
(-2.6470588235294117, 2.3199463508876157e-5)
(-2.607843137254902, 0.0001153966133340734)
(-2.568627450980392, 0.0002306038570493089)
(-2.5294117647058822, 0.00034895460046760024)
(-2.4901960784313726, 0.00037447028890270814)
(-2.450980392156863, 0.00034529419544211394)
(-2.411764705882353, 0.00032234468904397825)
(-2.372549019607843, 0.0003447690720798966)
(-2.3333333333333335, 0.0003222362444513007)
(-2.2941176470588234, 0.0004039679678153699)
(-2.2549019607843137, 0.0005239359098409105)
(-2.215686274509804, 0.0007754140009448967)
(-2.176470588235294, 0.0011537701128327958)
(-2.1372549019607843, 0.0014564442299740648)
(-2.0980392156862746, 0.00153917559257109)
(-2.0588235294117645, 0.001440740355310612)
(-2.019607843137255, 0.0014301550105656957)
(-1.9803921568627452, 0.0016345436344087961)
(-1.9411764705882353, 0.001645335514741804)
(-1.9019607843137254, 0.0013914712111046648)
(-1.8627450980392157, 0.0012668863418506759)
(-1.8235294117647058, 0.0017706622994447681)
(-1.784313725490196, 0.0025147697829376887)
(-1.7450980392156863, 0.0026575999368161334)
(-1.7058823529411764, 0.002026384087608558)
(-1.6666666666666667, 0.0021938983240872884)
(-1.6274509803921569, 0.0035417495993354253)
(-1.588235294117647, 0.003823116685511248)
(-1.5490196078431373, 0.0026262779406720817)
(-1.5098039215686274, 0.0008451835258271031)
(-1.4705882352941175, 0.002715643821216885)
(-1.4313725490196079, 0.004095396958311514)
(-1.392156862745098, 0.004434756312751441)
(-1.3529411764705883, 0.005174243134821081)
(-1.3137254901960784, 0.006742894502973343)
(-1.2745098039215685, 0.008777630628470624)
(-1.2352941176470589, 0.010656677519161627)
(-1.196078431372549, 0.012873064103375088)
(-1.156862745098039, 0.015567026348032108)
(-1.1176470588235294, 0.018335538929558966)
(-1.0784313725490196, 0.020699710655021762)
(-1.0392156862745099, 0.022428965089620247)
(-1.0, 0.023740708588019962)
(-0.9607843137254902, 0.02484487503043638)
(-0.9215686274509803, 0.025881453688999738)
(-0.8823529411764706, 0.026992313579590282)
(-0.8431372549019608, 0.028301889595343483)
(-0.803921568627451, 0.029865284141294492)
(-0.7647058823529411, 0.0316666281563707)
(-0.7254901960784313, 0.03367169332492953)
(-0.6862745098039216, 0.035871742089856155)
(-0.6470588235294118, 0.038289819929353125)
(-0.6078431372549019, 0.04097430557060224)
(-0.5686274509803921, 0.04399952335586438)
(-0.5294117647058824, 0.04747688378058397)
(-0.49019607843137253, 0.05157625200590075)
(-0.45098039215686275, 0.056561093914543434)
(-0.4117647058823529, 0.06284963457850405)
(-0.37254901960784315, 0.07112423058507676)
(-0.3333333333333333, 0.08252471705795399)
(-0.29411764705882354, 0.0989880582344854)
(-0.2549019607843137, 0.1238691444792711)
(-0.21568627450980393, 0.1631504393773947)
(-0.1764705882352941, 0.22762106797440562)
(-0.13725490196078433, 0.334808876134258)
(-0.09803921568627451, 0.5030050313427424)
(-0.058823529411764705, 0.7237420531476307)
(-0.0196078431372549, 0.9252019639732301)
(0.0196078431372549, 1.0)
(0.058823529411764705, 0.9117782947548126)
(0.09803921568627451, 0.7262604783512118)
(0.13725490196078433, 0.5296893373438918)
(0.1764705882352941, 0.3701375271544409)
(0.21568627450980393, 0.2576749957767012)
(0.2549019607843137, 0.18393225481653497)
(0.29411764705882354, 0.13681760478615432)
(0.3333333333333333, 0.10651565851262855)
(0.37254901960784315, 0.0864635633662378)
(0.4117647058823529, 0.07264651188904064)
(0.45098039215686275, 0.06269994364081405)
(0.49019607843137253, 0.05523882305060128)
(0.5294117647058824, 0.049438292283349325)
(0.5686274509803921, 0.044792134847612346)
(0.6078431372549019, 0.04097827008493239)
(0.6470588235294118, 0.037784147961513526)
(0.6862745098039216, 0.035064734203745465)
(0.7254901960784313, 0.03271817282532641)
(0.7647058823529411, 0.030671151988493683)
(0.803921568627451, 0.02886974685099674)
(0.8431372549019608, 0.02727353008570136)
(0.8823529411764706, 0.025851692761560466)
(0.9215686274509803, 0.0245799871154553)
(0.9607843137254902, 0.0234370679032836)
(1.0, 0.02239965744980901)
(1.0392156862745099, 0.021438421146327886)
(1.0784313725490196, 0.02051833712980375)
(1.1176470588235294, 0.019605360515923563)
(1.156862745098039, 0.018675776670825588)
(1.196078431372549, 0.01772068382382091)
(1.2352941176470589, 0.016738913883839746)
(1.2745098039215685, 0.015719858171506184)
(1.3137254901960784, 0.014631963295153615)
(1.3529411764705883, 0.013434470717911927)
(1.392156862745098, 0.01210764631566437)
(1.4313725490196079, 0.01067915412831606)
(1.4705882352941175, 0.009229648415667206)
(1.5098039215686274, 0.007870081029739757)
(1.5490196078431373, 0.006698319197523725)
(1.588235294117647, 0.005759822844282991)
(1.6274509803921569, 0.005030085731123559)
(1.6666666666666667, 0.00443287384892558)
(1.7058823529411764, 0.00388614956910856)
(1.7450980392156863, 0.003325544475670427)
(1.784313725490196, 0.002719333326994334)
(1.8235294117647058, 0.0021366133364638107)
(1.8627450980392157, 0.0017706358802901674)
(1.9019607843137254, 0.0016923108174588658)
(1.9411764705882353, 0.0016733868103245425)
(1.9803921568627452, 0.0014531492986223787)
(2.019607843137255, 0.000942425823119445)
(2.0588235294117645, 0.00028338673890064537)
(2.0980392156862746, 0.0002301852712780759)
(2.1372549019607843, 0.0003568927904631637)
(2.176470588235294, 4.882071344054014e-5)
(2.215686274509804, 0.0005615544198941374)
(2.2549019607843137, 0.0007757376491939927)
(2.2941176470588234, 0.0005282839027293307)
(2.3333333333333335, 0.00030928412396689984)
(2.372549019607843, 0.0005089345373942852)
(2.411764705882353, 0.0004850935221452762)
(2.450980392156863, 0.00041550313744873757)
(2.4901960784313726, 0.0003408159018479592)
(2.5294117647058822, 0.0002498238755289297)
(2.568627450980392, 0.0002804708614742967)
(2.607843137254902, 0.00035270697167901236)
(2.6470588235294117, 0.00034077728785228336)
(2.6862745098039214, 0.00022994874515529036)
(2.7254901960784315, 8.849995524068832e-5)
(2.764705882352941, 6.247613232454184e-5)
(2.803921568627451, 3.440746916824113e-5)
(2.843137254901961, 0.00011561815182409543)
(2.8823529411764706, 0.00016103051417019996)
(2.9215686274509802, 0.00016662143074811853)
(2.9607843137254903, 0.0001978862696792905)
(3.0, 0.00023238444930529097)
(3.0392156862745097, 0.0002784001642906013)
(3.0784313725490198, 0.0002869090922236652)
(3.1176470588235294, 0.00024250826668828116)
(3.156862745098039, 0.00021263867983860316)
(3.1960784313725488, 0.0001746517669183705)
(3.235294117647059, 0.0001151832468332008)
(3.2745098039215685, 8.054360391143554e-5)
(3.313725490196078, 6.941931554589376e-5)
(3.3529411764705883, 6.288934644840549e-5)
(3.392156862745098, 3.40602642957301e-5)
(3.4313725490196076, 2.3419289452596657e-5)
(3.4705882352941178, 2.3989183807352863e-5)
(3.5098039215686274, 1.951959060510803e-5)
(3.549019607843137, 3.0433346667584225e-5)
(3.588235294117647, 5.670804444521399e-5)
(3.627450980392157, 7.248362137961468e-5)
(3.6666666666666665, 7.7840644969333e-5)
(3.7058823529411766, 8.258792679762462e-5)
(3.7450980392156863, 7.720130057316165e-5)
(3.784313725490196, 7.048188697127384e-5)
(3.8235294117647056, 8.378264062246955e-5)
(3.8627450980392157, 7.360849165599917e-5)
(3.9019607843137254, 4.402074231980792e-5)
(3.941176470588235, 6.7269788117879e-5)
(3.980392156862745, 8.083628278169496e-5)
(4.019607843137255, 8.048479472275189e-5)
(4.0588235294117645, 8.058636585067299e-5)
(4.098039215686274, 5.8308948032950955e-5)
(4.137254901960784, 5.080109418583876e-5)
(4.176470588235294, 7.132084623191244e-5)
(4.215686274509804, 8.278956544946456e-5)
(4.254901960784314, 7.668979379408259e-5)
(4.294117647058823, 7.678374530340128e-5)
(4.333333333333333, 7.706129956625333e-5)
(4.372549019607843, 7.255391238696224e-5)
(4.411764705882353, 6.82825636423074e-5)
(4.450980392156863, 5.450136213425693e-5)
(4.490196078431373, 4.333812387413831e-5)
(4.529411764705882, 4.021255276459545e-5)
(4.568627450980392, 3.0455333279739133e-5)
(4.607843137254902, 3.355463536663282e-5)
(4.647058823529412, 3.193293983526706e-5)
(4.686274509803922, 3.0397998380557196e-5)
(4.7254901960784315, 2.920922307952592e-5)
(4.764705882352941, 1.6591881959076705e-5)
(4.803921568627451, 1.5979694850986778e-5)
(4.8431372549019605, 3.868725722012761e-5)
(4.88235294117647, 0.00010277831389008466)
(4.921568627450981, 0.00011086423097158153)
(4.96078431372549, 0.00012784737278968836)
(5.0, 0.00013378919715140448)
};

==> plots/das_azim_resol.tex <==
\addplot[very thick] coordinates {
(-5.0, 0.0003119665071269792)
(-4.96078431372549, 0.0004294110504484336)
(-4.921568627450981, 0.0004401070613824961)
(-4.88235294117647, 0.0004129614374156937)
(-4.8431372549019605, 0.000329887343481537)
(-4.803921568627451, 0.0002321148961750365)
(-4.764705882352941, 0.0001416098870690656)
(-4.7254901960784315, 0.00019380125340991998)
(-4.686274509803922, 0.000309049570105246)
(-4.647058823529412, 0.0003975742195470314)
(-4.607843137254902, 0.0004598209399615656)
(-4.568627450980392, 0.0004665028922019867)
(-4.529411764705882, 0.0004097121389119413)
(-4.490196078431373, 0.000304194679033673)
(-4.450980392156863, 0.00023941436416374898)
(-4.411764705882353, 0.0003613969614653693)
(-4.372549019607843, 0.0005794708284923203)
(-4.333333333333333, 0.0007863402002104358)
(-4.294117647058823, 0.0009315327583273853)
(-4.254901960784314, 0.0009885934415569011)
(-4.215686274509804, 0.0009530401273109109)
(-4.176470588235294, 0.0008422255403235313)
(-4.137254901960784, 0.0006895667445506029)
(-4.098039215686274, 0.0005342710309698528)
(-4.0588235294117645, 0.00040197797879320727)
(-4.019607843137255, 0.00028755810266484216)
(-3.980392156862745, 0.00016024674364550147)
(-3.941176470588235, 3.087939617407435e-5)
(-3.9019607843137254, 0.0002157151585640235)
(-3.8627450980392157, 0.0004345199143223512)
(-3.8235294117647056, 0.0006353567393368506)
(-3.784313725490196, 0.0007817053402773438)
(-3.7450980392156863, 0.0008455136917820214)
(-3.7058823529411766, 0.0008123719893124149)
(-3.6666666666666665, 0.0006896458536723354)
(-3.627450980392157, 0.0005194668245653861)
(-3.588235294117647, 0.00042359699056272526)
(-3.549019607843137, 0.0005489645815574323)
(-3.5098039215686274, 0.0008021119966142831)
(-3.4705882352941178, 0.0010615868206620166)
(-3.4313725490196076, 0.0012794270842691868)
(-3.392156862745098, 0.0014446132139683797)
(-3.3529411764705883, 0.0015681616995894025)
(-3.313725490196078, 0.0016716231638748856)
(-3.2745098039215685, 0.001774674522328814)
(-3.235294117647059, 0.0018845820267474151)
(-3.1960784313725488, 0.0019991230403968692)
(-3.156862745098039, 0.002119387484668384)
(-3.1176470588235294, 0.0022588216732068087)
(-3.0784313725490198, 0.0024464769978278125)
(-3.0392156862745097, 0.002710302557116077)
(-3.0, 0.0030598471955649016)
(-2.9607843137254903, 0.003480244012270986)
(-2.9215686274509802, 0.003942531425481441)
(-2.8823529411764706, 0.004418729387027041)
(-2.843137254901961, 0.004890276205987571)
(-2.803921568627451, 0.005351873055133713)
(-2.764705882352941, 0.005808933751510971)
(-2.7254901960784315, 0.006274217233521178)
(-2.6862745098039214, 0.006761534302278229)
(-2.6470588235294117, 0.007289796747507603)
(-2.607843137254902, 0.00787788184385936)
(-2.568627450980392, 0.008546909584722985)
(-2.5294117647058822, 0.009313278383950767)
(-2.4901960784313726, 0.010182242652926186)
(-2.450980392156863, 0.011146180260850467)
(-2.411764705882353, 0.012179871382636426)
(-2.372549019607843, 0.01325244646330367)
(-2.3333333333333335, 0.014335258261743257)
(-2.2941176470588234, 0.015409943600446152)
(-2.2549019607843137, 0.016480201569805345)
(-2.215686274509804, 0.017567608153219602)
(-2.176470588235294, 0.018710776713808126)
(-2.1372549019607843, 0.019957792517160337)
(-2.0980392156862746, 0.021353201379406807)
(-2.0588235294117645, 0.022932613204130776)
(-2.019607843137255, 0.024719256602113136)
(-1.9803921568627452, 0.02672598613169658)
(-1.9411764705882353, 0.02895692881394743)
(-1.9019607843137254, 0.0314128976100582)
(-1.8627450980392157, 0.03409805825725666)
(-1.8235294117647058, 0.037023039667514426)
(-1.784313725490196, 0.040218814499528195)
(-1.7450980392156863, 0.043759177449738756)
(-1.7058823529411764, 0.04778371663925039)
(-1.6666666666666667, 0.0525234486079144)
(-1.6274509803921569, 0.05831769984707873)
(-1.588235294117647, 0.06560203556302771)
(-1.5490196078431373, 0.074861548283632)
(-1.5098039215686274, 0.08656330663724682)
(-1.4705882352941175, 0.10109297312604518)
(-1.4313725490196079, 0.11871634910836368)
(-1.392156862745098, 0.13956935318261582)
(-1.3529411764705883, 0.16366614729399578)
(-1.3137254901960784, 0.1909148742710612)
(-1.2745098039215685, 0.22113557252774962)
(-1.2352941176470589, 0.25407620171871376)
(-1.196078431372549, 0.2894244752699933)
(-1.156862745098039, 0.3268183090461741)
(-1.1176470588235294, 0.36585893503259564)
(-1.0784313725490196, 0.40612570361161304)
(-1.0392156862745099, 0.44718843123769286)
(-1.0, 0.48861639161945486)
(-0.9607843137254902, 0.5299869777870077)
(-0.9215686274509803, 0.5708960767048864)
(-0.8823529411764706, 0.6109683487758193)
(-0.8431372549019608, 0.6498644231306737)
(-0.803921568627451, 0.6872843846568595)
(-0.7647058823529411, 0.7229693896628127)
(-0.7254901960784313, 0.756703169740566)
(-0.6862745098039216, 0.7883134867692825)
(-0.6470588235294118, 0.817672535779402)
(-0.6078431372549019, 0.8446955740974176)
(-0.5686274509803921, 0.8693378749245344)
(-0.5294117647058824, 0.8915906617167322)
(-0.49019607843137253, 0.9114767237259023)
(-0.45098039215686275, 0.9290461357354579)
(-0.4117647058823529, 0.9443721920411257)
(-0.37254901960784315, 0.9575474806798312)
(-0.3333333333333333, 0.9686800010294415)
(-0.29411764705882354, 0.97788930358979)
(-0.2549019607843137, 0.9853026872402156)
(-0.21568627450980393, 0.9910515683129235)
(-0.1764705882352941, 0.9952681591082263)
(-0.13725490196078433, 0.9980825495575143)
(-0.09803921568627451, 0.9996202247284977)
(-0.058823529411764705, 1.0)
(-0.0196078431372549, 0.9993323298039709)
(0.0196078431372549, 0.9977179425407913)
(0.058823529411764705, 0.9952467629665918)
(0.09803921568627451, 0.9919970928298524)
(0.13725490196078433, 0.9880350274273632)
(0.1764705882352941, 0.9834140898955294)
(0.21568627450980393, 0.9781750674106886)
(0.2549019607843137, 0.9723460351710602)
(0.29411764705882354, 0.9659425558293345)
(0.3333333333333333, 0.9589680442296447)
(0.37254901960784315, 0.9514142897851885)
(0.4117647058823529, 0.9432621313725715)
(0.45098039215686275, 0.9344822818951659)
(0.49019607843137253, 0.9250363014807056)
(0.5294117647058824, 0.9148777195842537)
(0.5686274509803921, 0.9039533071837911)
(0.6078431372549019, 0.8922045011244755)
(0.6470588235294118, 0.8795689837729336)
(0.6862745098039216, 0.8659824224135882)
(0.7254901960784313, 0.8513803733334551)
(0.7647058823529411, 0.8357003533987812)
(0.803921568627451, 0.8188840733584362)
(0.8431372549019608, 0.8008798108462201)
(0.8823529411764706, 0.781644875421555)
(0.9215686274509803, 0.7611480909696137)
(0.9607843137254902, 0.7393722008032253)
(1.0, 0.7163161041187972)
(1.0392156862745099, 0.691996862864171)
(1.0784313725490196, 0.666451466325443)
(1.1176470588235294, 0.6397383712159137)
(1.156862745098039, 0.6119387990462938)
(1.196078431372549, 0.5831576536886329)
(1.2352941176470589, 0.5535237931826267)
(1.2745098039215685, 0.5231893825146154)
(1.3137254901960784, 0.4923282355960097)
(1.3529411764705883, 0.4611332956046847)
(1.392156862745098, 0.4298134702689127)
(1.4313725490196079, 0.39858985423173365)
(1.4705882352941175, 0.367691205250646)
(1.5098039215686274, 0.33734865747225584)
(1.5490196078431373, 0.3077898867993979)
(1.588235294117647, 0.2792329483554794)
(1.6274509803921569, 0.2518799436236341)
(1.6666666666666667, 0.22591089491102032)
(1.7058823529411764, 0.20147856540587447)
(1.7450980392156863, 0.17870470866001806)
(1.784313725490196, 0.15767748692616448)
(1.8235294117647058, 0.13844974670129678)
(1.8627450980392157, 0.1210389238030851)
(1.9019607843137254, 0.10542966314845575)
(1.9411764705882353, 0.09157834292843425)
(1.9803921568627452, 0.07941724223520336)
(2.019607843137255, 0.06885771660035417)
(2.0588235294117645, 0.05979335634022625)
(2.0980392156862746, 0.052102521667812124)
(2.1372549019607843, 0.045648620518422604)
(2.176470588235294, 0.04027924378722396)
(2.215686274509804, 0.0358281250260031)
(2.2549019607843137, 0.03212256363260016)
(2.2941176470588234, 0.028995317962199136)
(2.3333333333333335, 0.026298164594199445)
(2.372549019607843, 0.02391351464251117)
(2.411764705882353, 0.021761224420002404)
(2.450980392156863, 0.019799562191139892)
(2.4901960784313726, 0.018017907482705525)
(2.5294117647058822, 0.016423539255837765)
(2.568627450980392, 0.015028861236229842)
(2.607843137254902, 0.013836862135810146)
(2.6470588235294117, 0.012829583487091008)
(2.6862745098039214, 0.011967974978063081)
(2.7254901960784315, 0.011198450105840288)
(2.764705882352941, 0.01046463691580513)
(2.803921568627451, 0.009719776305513635)
(2.843137254901961, 0.00893513096309652)
(2.8823529411764706, 0.008102369197624087)
(2.9215686274509802, 0.007234001470386375)
(2.9607843137254903, 0.006363746947134702)
(3.0, 0.005541877609000275)
(3.0392156862745097, 0.004832236673948458)
(3.0784313725490198, 0.004296749055282148)
(3.1176470588235294, 0.0039665801422297895)
(3.156862745098039, 0.0038154149284962487)
(3.1960784313725488, 0.0037611747480617015)
(3.235294117647059, 0.0037075012834046537)
(3.2745098039215685, 0.003579423597864746)
(3.313725490196078, 0.003336892809296604)
(3.3529411764705883, 0.0029759604366000505)
(3.392156862745098, 0.0025221046635391666)
(3.4313725490196076, 0.0020260282197110033)
(3.4705882352941178, 0.001559367014053036)
(3.5098039215686274, 0.0012113572060704096)
(3.549019607843137, 0.0010540823221554371)
(3.588235294117647, 0.0010592000538358164)
(3.627450980392157, 0.001112907743215758)
(3.6666666666666665, 0.0011327231187287174)
(3.7058823529411766, 0.0010934506073946553)
(3.7450980392156863, 0.0010045292496473812)
(3.784313725490196, 0.0008892653427852448)
(3.8235294117647056, 0.0007697045486979475)
(3.8627450980392157, 0.000656089677474745)
(3.9019607843137254, 0.0005496558931994191)
(3.941176470588235, 0.0004581870170937157)
(3.980392156862745, 0.0004187927427087481)
(4.019607843137255, 0.00047677859277558087)
(4.0588235294117645, 0.0006136973549318168)
(4.098039215686274, 0.0007716957249843292)
(4.137254901960784, 0.0009043194410701911)
(4.176470588235294, 0.0009821642371424862)
(4.215686274509804, 0.0009905287789460048)
(4.254901960784314, 0.0009275234798410383)
(4.294117647058823, 0.0008033248582080155)
(4.333333333333333, 0.0006369422786246704)
(4.372549019607843, 0.00045141029158705655)
(4.411764705882353, 0.00027167566488615446)
(4.450980392156863, 0.00011996209088864443)
(4.490196078431373, 4.6796198713890046e-5)
(4.529411764705882, 9.316240193087968e-5)
(4.568627450980392, 0.00011679489329370956)
(4.607843137254902, 0.00010323150078848514)
(4.647058823529412, 8.129052239269577e-5)
(4.686274509803922, 0.00013097992791267617)
(4.7254901960784315, 0.00024294675764539931)
(4.764705882352941, 0.0003751535532237419)
(4.803921568627451, 0.0005054282339864171)
(4.8431372549019605, 0.000616650476616353)
(4.88235294117647, 0.000696107996853204)
(4.921568627450981, 0.0007364590219737504)
(4.96078431372549, 0.0007352733381998349)
(5.0, 0.0006954540230822689)
};

==> plots/lml_8_azim_resol.tex <==
\addplot[very thick,color=color4] coordinates {
(-5.0, 2.598697339608795e-9)
(-4.96078431372549, 2.5986993882079807e-9)
(-4.921568627450981, 2.5987008343804238e-9)
(-4.88235294117647, 2.5987006584693033e-9)
(-4.8431372549019605, 2.598698859643337e-9)
(-4.803921568627451, 2.5986966167308474e-9)
(-4.764705882352941, 2.598695398997095e-9)
(-4.7254901960784315, 2.5986959471928216e-9)
(-4.686274509803922, 2.5986981619799894e-9)
(-4.647058823529412, 2.5987007045006032e-9)
(-4.607843137254902, 2.598701392712893e-9)
(-4.568627450980392, 2.5987002199246383e-9)
(-4.529411764705882, 2.598697856716137e-9)
(-4.490196078431373, 2.5986956351583466e-9)
(-4.450980392156863, 2.598695068780747e-9)
(-4.411764705882353, 2.5986971830369928e-9)
(-4.372549019607843, 2.5987006744932083e-9)
(-4.333333333333333, 2.5987062197029985e-9)
(-4.294117647058823, 2.5987118848428266e-9)
(-4.254901960784314, 2.598715148462258e-9)
(-4.215686274509804, 2.5987156194597603e-9)
(-4.176470588235294, 2.598713030227853e-9)
(-4.137254901960784, 2.598709104168302e-9)
(-4.098039215686274, 2.5987051589040746e-9)
(-4.0588235294117645, 2.598702240386147e-9)
(-4.019607843137255, 2.598700621995841e-9)
(-3.980392156862745, 2.598700235093331e-9)
(-3.941176470588235, 2.5987008359864714e-9)
(-3.9019607843137254, 2.598702225322536e-9)
(-3.8627450980392157, 2.598704217812603e-9)
(-3.8235294117647056, 2.5987065086168415e-9)
(-3.784313725490196, 2.598708712581793e-9)
(-3.7450980392156863, 2.598710362005811e-9)
(-3.7058823529411766, 2.5987110676084215e-9)
(-3.6666666666666665, 2.598710503513225e-9)
(-3.627450980392157, 2.5987086449598566e-9)
(-3.588235294117647, 2.5987058847306053e-9)
(-3.549019607843137, 2.5987029767420505e-9)
(-3.5098039215686274, 2.5987008836147742e-9)
(-3.4705882352941178, 2.5987005386217827e-9)
(-3.4313725490196076, 2.598702739264693e-9)
(-3.392156862745098, 2.598707559889817e-9)
(-3.3529411764705883, 2.5987145310091303e-9)
(-3.313725490196078, 2.5987229064140255e-9)
(-3.2745098039215685, 2.5987314671949564e-9)
(-3.235294117647059, 2.5987396047941204e-9)
(-3.1960784313725488, 2.5987463825203105e-9)
(-3.156862745098039, 2.598751132814278e-9)
(-3.1176470588235294, 2.5987540798114073e-9)
(-3.0784313725490198, 2.5987553123330065e-9)
(-3.0392156862745097, 2.598756170123217e-9)
(-3.0, 2.5987574294525224e-9)
(-2.9607843137254903, 2.5987596883316593e-9)
(-2.9215686274509802, 2.598763238304805e-9)
(-2.8823529411764706, 2.5987672902751325e-9)
(-2.843137254901961, 2.5987706097864254e-9)
(-2.803921568627451, 2.598771846632803e-9)
(-2.764705882352941, 2.598771942979799e-9)
(-2.7254901960784315, 2.598771282841649e-9)
(-2.6862745098039214, 2.598771381519786e-9)
(-2.6470588235294117, 2.5987749371342156e-9)
(-2.607843137254902, 2.59878232961208e-9)
(-2.568627450980392, 2.5987938671461706e-9)
(-2.5294117647058822, 2.59880950140767e-9)
(-2.4901960784313726, 2.5988272805887095e-9)
(-2.450980392156863, 2.5988505861162058e-9)
(-2.411764705882353, 2.5988777193485194e-9)
(-2.372549019607843, 2.5989126651394906e-9)
(-2.3333333333333335, 2.5989585525765136e-9)
(-2.2941176470588234, 2.5990232366593558e-9)
(-2.2549019607843137, 2.599101470603045e-9)
(-2.215686274509804, 2.5992014927592178e-9)
(-2.176470588235294, 2.5993270726359425e-9)
(-2.1372549019607843, 2.5994659809365403e-9)
(-2.0980392156862746, 2.599617378966604e-9)
(-2.0588235294117645, 2.5998007220588872e-9)
(-2.019607843137255, 2.6000269351837845e-9)
(-1.9803921568627452, 2.600239659650461e-9)
(-1.9411764705882353, 2.6004428376440676e-9)
(-1.9019607843137254, 2.600793475777895e-9)
(-1.8627450980392157, 2.601266968606313e-9)
(-1.8235294117647058, 2.601648051574491e-9)
(-1.784313725490196, 2.60203989192961e-9)
(-1.7450980392156863, 2.602749497994237e-9)
(-1.7058823529411764, 2.60382092006674e-9)
(-1.6666666666666667, 2.604971779869856e-9)
(-1.6274509803921569, 2.6061062541518195e-9)
(-1.588235294117647, 2.6079551313179227e-9)
(-1.5490196078431373, 2.6115791431474976e-9)
(-1.5098039215686274, 2.6170689482339454e-9)
(-1.4705882352941175, 2.6239535233107947e-9)
(-1.4313725490196079, 2.6336507306531795e-9)
(-1.392156862745098, 2.64922301652467e-9)
(-1.3529411764705883, 2.672334745376697e-9)
(-1.3137254901960784, 2.7042497477916705e-9)
(-1.2745098039215685, 2.746487207246513e-9)
(-1.2352941176470589, 2.8028137730990183e-9)
(-1.196078431372549, 2.87683018158093e-9)
(-1.156862745098039, 2.9708183479717446e-9)
(-1.1176470588235294, 3.086632301307791e-9)
(-1.0784313725490196, 3.2255527512681427e-9)
(-1.0392156862745099, 3.3881871069841014e-9)
(-1.0, 3.5750966288907445e-9)
(-0.9607843137254902, 3.786964883236046e-9)
(-0.9215686274509803, 4.0256888250350266e-9)
(-0.8823529411764706, 4.295515970239771e-9)
(-0.8431372549019608, 4.604236404432586e-9)
(-0.803921568627451, 4.964652439102757e-9)
(-0.7647058823529411, 5.396290725238178e-9)
(-0.7254901960784313, 5.927824131372046e-9)
(-0.6862745098039216, 6.601336221029954e-9)
(-0.6470588235294118, 7.480407640762178e-9)
(-0.6078431372549019, 8.665477928786164e-9)
(-0.5686274509803921, 1.0323437107747477e-8)
(-0.5294117647058824, 1.2747435103544306e-8)
(-0.49019607843137253, 1.64864782263537e-8)
(-0.45098039215686275, 2.2650858879734887e-8)
(-0.4117647058823529, 3.370763952905253e-8)
(-0.37254901960784315, 5.581940097098578e-8)
(-0.3333333333333333, 1.0683221697345287e-7)
(-0.29411764705882354, 2.492136757323262e-7)
(-0.2549019607843137, 7.626884624287667e-7)
(-0.21568627450980393, 3.3742887551587247e-6)
(-0.1764705882352941, 2.41489695751262e-5)
(-0.13725490196078433, 0.0003039067018738503)
(-0.09803921568627451, 0.006239135730695381)
(-0.058823529411764705, 0.12989515197626283)
(-0.0196078431372549, 0.9934798232527585)
(0.0196078431372549, 1.0)
(0.058823529411764705, 0.13072085851064497)
(0.09803921568627451, 0.006136373526394734)
(0.13725490196078433, 0.0002894361059172095)
(0.1764705882352941, 2.238420861367978e-5)
(0.21568627450980393, 3.073324894012134e-6)
(0.2549019607843137, 6.881669335904648e-7)
(0.29411764705882354, 2.24024475550708e-7)
(0.3333333333333333, 9.603619040852717e-8)
(0.37254901960784315, 5.0306281136477165e-8)
(0.4117647058823529, 3.050820166534269e-8)
(0.45098039215686275, 2.061287069781212e-8)
(0.49019607843137253, 1.509755367357498e-8)
(0.5294117647058824, 1.1754062722862887e-8)
(0.5686274509803921, 9.589211793098399e-9)
(0.6078431372549019, 8.11198202347643e-9)
(0.6470588235294118, 7.0601450963066245e-9)
(0.6862745098039216, 6.284422013147597e-9)
(0.7254901960784313, 5.695157643406921e-9)
(0.7647058823529411, 5.23600370749563e-9)
(0.803921568627451, 4.870139129111513e-9)
(0.8431372549019608, 4.572678970843433e-9)
(0.8823529411764706, 4.326306068111495e-9)
(0.9215686274509803, 4.11866464556413e-9)
(0.9607843137254902, 3.9407624552272205e-9)
(1.0, 3.785972631075898e-9)
(1.0392156862745099, 3.6493978997887596e-9)
(1.0784313725490196, 3.527447494029625e-9)
(1.1176470588235294, 3.4175296873270634e-9)
(1.156862745098039, 3.3178069900973155e-9)
(1.196078431372549, 3.2269988676698416e-9)
(1.2352941176470589, 3.1442356227694365e-9)
(1.2745098039215685, 3.0689555223555883e-9)
(1.3137254901960784, 3.000814491140949e-9)
(1.3529411764705883, 2.9395830034012463e-9)
(1.392156862745098, 2.8850441855410457e-9)
(1.4313725490196079, 2.8369325740137844e-9)
(1.4705882352941175, 2.7949281130610485e-9)
(1.5098039215686274, 2.7586743744255554e-9)
(1.5490196078431373, 2.727779724473556e-9)
(1.588235294117647, 2.7017941356681518e-9)
(1.6274509803921569, 2.680198758055353e-9)
(1.6666666666666667, 2.6624461310309607e-9)
(1.7058823529411764, 2.648020242521516e-9)
(1.7450980392156863, 2.6364597097207963e-9)
(1.784313725490196, 2.6273283117205576e-9)
(1.8235294117647058, 2.620185313469417e-9)
(1.8627450980392157, 2.6146368122876983e-9)
(1.9019607843137254, 2.6103997677009222e-9)
(1.9411764705882353, 2.6072604055401915e-9)
(1.9803921568627452, 2.6049855316184155e-9)
(2.019607843137255, 2.6033228311006362e-9)
(2.0588235294117645, 2.6020896806281108e-9)
(2.0980392156862746, 2.6012146681236726e-9)
(2.1372549019607843, 2.600662218375556e-9)
(2.176470588235294, 2.6003200093396847e-9)
(2.215686274509804, 2.6000322594780853e-9)
(2.2549019607843137, 2.5997777951524362e-9)
(2.2941176470588234, 2.5996393877670887e-9)
(2.3333333333333335, 2.5995672145298463e-9)
(2.372549019607843, 2.5994537622626954e-9)
(2.411764705882353, 2.5993243329178438e-9)
(2.450980392156863, 2.599245015463379e-9)
(2.4901960784313726, 2.59918826439616e-9)
(2.5294117647058822, 2.5991174348465326e-9)
(2.568627450980392, 2.5990518668767425e-9)
(2.607843137254902, 2.599002800462161e-9)
(2.6470588235294117, 2.5989533293921357e-9)
(2.6862745098039214, 2.59890946797848e-9)
(2.7254901960784315, 2.5988735522226753e-9)
(2.764705882352941, 2.598844058164353e-9)
(2.803921568627451, 2.598819840042464e-9)
(2.843137254901961, 2.5988027968242847e-9)
(2.8823529411764706, 2.5987950613001783e-9)
(2.9215686274509802, 2.5987881230829085e-9)
(2.9607843137254903, 2.59878594399217e-9)
(3.0, 2.5987842756523346e-9)
(3.0392156862745097, 2.598781488176885e-9)
(3.0784313725490198, 2.598776678032378e-9)
(3.1176470588235294, 2.5987683952764257e-9)
(3.156862745098039, 2.598759072064685e-9)
(3.1960784313725488, 2.5987475034524657e-9)
(3.235294117647059, 2.5987372286609794e-9)
(3.2745098039215685, 2.5987290427839934e-9)
(3.313725490196078, 2.598722985529794e-9)
(3.3529411764705883, 2.598719193140813e-9)
(3.392156862745098, 2.5987174627449043e-9)
(3.4313725490196076, 2.5987166760260692e-9)
(3.4705882352941178, 2.5987170328752592e-9)
(3.5098039215686274, 2.598718801977544e-9)
(3.549019607843137, 2.5987213464127244e-9)
(3.588235294117647, 2.5987241700121174e-9)
(3.627450980392157, 2.5987261821183696e-9)
(3.6666666666666665, 2.598725985529625e-9)
(3.7058823529411766, 2.5987235071044733e-9)
(3.7450980392156863, 2.5987190712319822e-9)
(3.784313725490196, 2.5987137396052435e-9)
(3.8235294117647056, 2.598708641313161e-9)
(3.8627450980392157, 2.598704227618732e-9)
(3.9019607843137254, 2.59870057817237e-9)
(3.941176470588235, 2.5986981330749764e-9)
(3.980392156862745, 2.5986968595383003e-9)
(4.019607843137255, 2.598697306395719e-9)
(4.0588235294117645, 2.598699022225721e-9)
(4.098039215686274, 2.5987017948725943e-9)
(4.137254901960784, 2.5987046996411996e-9)
(4.176470588235294, 2.5987075222421654e-9)
(4.215686274509804, 2.5987093908728588e-9)
(4.254901960784314, 2.598710044536997e-9)
(4.294117647058823, 2.5987091563437103e-9)
(4.333333333333333, 2.598707054131007e-9)
(4.372549019607843, 2.5987041385946855e-9)
(4.411764705882353, 2.5987009577151525e-9)
(4.450980392156863, 2.5986979372656135e-9)
(4.490196078431373, 2.5986954173406503e-9)
(4.529411764705882, 2.598693671669756e-9)
(4.568627450980392, 2.5986925699666993e-9)
(4.607843137254902, 2.598692199232334e-9)
(4.647058823529412, 2.5986923266418383e-9)
(4.686274509803922, 2.59869287307636e-9)
(4.7254901960784315, 2.5986939894633885e-9)
(4.764705882352941, 2.598695403721528e-9)
(4.803921568627451, 2.5986976428071544e-9)
(4.8431372549019605, 2.5987003159404704e-9)
(4.88235294117647, 2.5987033030892073e-9)
(4.921568627450981, 2.598706677551637e-9)
(4.96078431372549, 2.5987090444364875e-9)
(5.0, 2.59871012795455e-9)
};

==> plots/mv_azim_resol.tex <==
\addplot[very thick,color=color1] coordinates {
(-5.0, 0.00027265718314112254)
(-4.96078431372549, 0.00041563220114430394)
(-4.921568627450981, 0.0004114122658265841)
(-4.88235294117647, 0.0003231833666583546)
(-4.8431372549019605, 0.00021154112907356985)
(-4.803921568627451, 7.669058662656991e-5)
(-4.764705882352941, 7.128868100555043e-5)
(-4.7254901960784315, 0.00022716343911427457)
(-4.686274509803922, 0.00039009521605785577)
(-4.647058823529412, 0.00047318063073523294)
(-4.607843137254902, 0.0005159756743376918)
(-4.568627450980392, 0.00048806013490058887)
(-4.529411764705882, 0.00035643548086023173)
(-4.490196078431373, 0.00023012748648655552)
(-4.450980392156863, 0.00014241317869737773)
(-4.411764705882353, 0.0002444162027092508)
(-4.372549019607843, 0.00031622865567066663)
(-4.333333333333333, 0.0004115355576672413)
(-4.294117647058823, 0.0005686625884934203)
(-4.254901960784314, 0.0006566445583931676)
(-4.215686274509804, 0.0006578135364177708)
(-4.176470588235294, 0.0005995241431689252)
(-4.137254901960784, 0.0005267840281601025)
(-4.098039215686274, 0.0004515998349290993)
(-4.0588235294117645, 0.00038631377083686406)
(-4.019607843137255, 0.0003404738971842664)
(-3.980392156862745, 0.0002976400554296047)
(-3.941176470588235, 0.00023482919055367097)
(-3.9019607843137254, 0.00019321978967180338)
(-3.8627450980392157, 0.00023462735819771043)
(-3.8235294117647056, 0.00032779368607187634)
(-3.784313725490196, 0.0004366607164923191)
(-3.7450980392156863, 0.0005253092446642568)
(-3.7058823529411766, 0.0005904047701385562)
(-3.6666666666666665, 0.0006188600797644138)
(-3.627450980392157, 0.0005897751810769351)
(-3.588235294117647, 0.000503693708616898)
(-3.549019607843137, 0.00037799936680816035)
(-3.5098039215686274, 0.000225588811055832)
(-3.4705882352941178, 6.81344281869498e-5)
(-3.4313725490196076, 0.000160653066885306)
(-3.392156862745098, 0.0003642060238383153)
(-3.3529411764705883, 0.0005362101196255782)
(-3.313725490196078, 0.0006492077006192818)
(-3.2745098039215685, 0.0007208455275029912)
(-3.235294117647059, 0.0007556440368392516)
(-3.1960784313725488, 0.0007689227694548668)
(-3.156862745098039, 0.0007582033407092497)
(-3.1176470588235294, 0.0007406533210428872)
(-3.0784313725490198, 0.000709731369438342)
(-3.0392156862745097, 0.0006557030163515293)
(-3.0, 0.000581394048917552)
(-2.9607843137254903, 0.0004412034837680309)
(-2.9215686274509802, 0.0002515890579302492)
(-2.8823529411764706, 0.00020905501136219331)
(-2.843137254901961, 0.00031475843769483757)
(-2.803921568627451, 0.0004126430872691883)
(-2.764705882352941, 0.00045079312062441335)
(-2.7254901960784315, 0.0004833811229370558)
(-2.6862745098039214, 0.0005114389311661291)
(-2.6470588235294117, 0.0005475170789727853)
(-2.607843137254902, 0.0006097881309109979)
(-2.568627450980392, 0.0007200170365153377)
(-2.5294117647058822, 0.0007889173592796321)
(-2.4901960784313726, 0.0008462699784596183)
(-2.450980392156863, 0.0008770915128286115)
(-2.411764705882353, 0.0009241877547648028)
(-2.372549019607843, 0.0009631100441967666)
(-2.3333333333333335, 0.0010613137093776533)
(-2.2941176470588234, 0.0013063281796575632)
(-2.2549019607843137, 0.0016974786598461945)
(-2.215686274509804, 0.002112243052354745)
(-2.176470588235294, 0.002445263916447518)
(-2.1372549019607843, 0.002710048339440772)
(-2.0980392156862746, 0.0029615793075392534)
(-2.0588235294117645, 0.003168485500998831)
(-2.019607843137255, 0.003285223067663483)
(-1.9803921568627452, 0.0031969306210353357)
(-1.9411764705882353, 0.002787955892720294)
(-1.9019607843137254, 0.0025042053142948933)
(-1.8627450980392157, 0.002848155289628504)
(-1.8235294117647058, 0.0038393663301936006)
(-1.784313725490196, 0.004798100298495902)
(-1.7450980392156863, 0.005408928399446228)
(-1.7058823529411764, 0.005672440117681708)
(-1.6666666666666667, 0.005798107903197014)
(-1.6274509803921569, 0.0053922354736001725)
(-1.588235294117647, 0.0036307629323915265)
(-1.5490196078431373, 0.002131047948215403)
(-1.5098039215686274, 0.00284498043423584)
(-1.4705882352941175, 0.004342473975659805)
(-1.4313725490196079, 0.006919092391790659)
(-1.392156862745098, 0.010017462352016086)
(-1.3529411764705883, 0.01351451282848229)
(-1.3137254901960784, 0.01747590753234197)
(-1.2745098039215685, 0.022087500737274186)
(-1.2352941176470589, 0.027756505583393074)
(-1.196078431372549, 0.03518767063728984)
(-1.156862745098039, 0.04514679319743838)
(-1.1176470588235294, 0.057915994316949014)
(-1.0784313725490196, 0.07292552691245548)
(-1.0392156862745099, 0.08895191114310594)
(-1.0, 0.10468238241153686)
(-0.9607843137254902, 0.11915358027835564)
(-0.9215686274509803, 0.13188225860131986)
(-0.8823529411764706, 0.14279299690501293)
(-0.8431372549019608, 0.15205408010857566)
(-0.803921568627451, 0.1599201358432174)
(-0.7647058823529411, 0.16664927719568434)
(-0.7254901960784313, 0.17248289228865826)
(-0.6862745098039216, 0.17764444262095688)
(-0.6470588235294118, 0.18234156312319239)
(-0.6078431372549019, 0.18677747042451506)
(-0.5686274509803921, 0.19117685650166552)
(-0.5294117647058824, 0.19582796644946868)
(-0.49019607843137253, 0.2011449190657721)
(-0.45098039215686275, 0.20776030705220808)
(-0.4117647058823529, 0.2166632148721226)
(-0.37254901960784315, 0.2293969126166033)
(-0.3333333333333333, 0.24831663134893134)
(-0.29411764705882354, 0.27687216131346426)
(-0.2549019607843137, 0.3198232209174178)
(-0.21568627450980393, 0.3832116538632907)
(-0.1764705882352941, 0.473675135286881)
(-0.13725490196078433, 0.5959295835389211)
(-0.09803921568627451, 0.7459379993092229)
(-0.058823529411764705, 0.8984085517524935)
(-0.0196078431372549, 1.0)
(0.0196078431372549, 0.9977208382410335)
(0.058823529411764705, 0.8923517546874153)
(0.09803921568627451, 0.7378117963687097)
(0.13725490196078433, 0.5873123882924586)
(0.1764705882352941, 0.46552218240748694)
(0.21568627450980393, 0.3758712241306549)
(0.2549019607843137, 0.31321215275517017)
(0.29411764705882354, 0.2706572398819278)
(0.3333333333333333, 0.24207170727402982)
(0.37254901960784315, 0.2227199778945301)
(0.4117647058823529, 0.20924168069559593)
(0.45098039215686275, 0.19939193751180873)
(0.49019607843137253, 0.19173396106652058)
(0.5294117647058824, 0.18537351664340374)
(0.5686274509803921, 0.1797629483669475)
(0.6078431372549019, 0.17456904346634397)
(0.6470588235294118, 0.16958829668654363)
(0.6862745098039216, 0.16469384712744173)
(0.7254901960784313, 0.1598024338359)
(0.7647058823529411, 0.15485369590175307)
(0.803921568627451, 0.14979713756804353)
(0.8431372549019608, 0.14458411387298586)
(0.8823529411764706, 0.13916342580284163)
(0.9215686274509803, 0.13347979012487787)
(0.9607843137254902, 0.12747475692091587)
(1.0, 0.12108967928189901)
(1.0392156862745099, 0.1142704263589017)
(1.0784313725490196, 0.10697406411556448)
(1.1176470588235294, 0.099178690670199)
(1.156862745098039, 0.09089812664221648)
(1.196078431372549, 0.0822014480194626)
(1.2352941176470589, 0.07323274810651)
(1.2745098039215685, 0.06422252788221046)
(1.3137254901960784, 0.05548208630195418)
(1.3529411764705883, 0.04737228363137671)
(1.392156862745098, 0.04023735555936189)
(1.4313725490196079, 0.034308857524193735)
(1.4705882352941175, 0.02961888208660258)
(1.5098039215686274, 0.025980160536525382)
(1.5490196078431373, 0.023064164756835485)
(1.588235294117647, 0.020542227320789034)
(1.6274509803921569, 0.0181981453296031)
(1.6666666666666667, 0.01594898494223815)
(1.7058823529411764, 0.013797427715471112)
(1.7450980392156863, 0.011776118289973167)
(1.784313725490196, 0.00991103816821937)
(1.8235294117647058, 0.008204449691305862)
(1.8627450980392157, 0.006637578780387921)
(1.9019607843137254, 0.005177341515069882)
(1.9411764705882353, 0.0037923502570725316)
(1.9803921568627452, 0.002508241765134861)
(2.019607843137255, 0.0014652147804849523)
(2.0588235294117645, 0.0009220235337158526)
(2.0980392156862746, 0.0008543664986772938)
(2.1372549019607843, 0.0007456449786373249)
(2.176470588235294, 0.0005412093914193336)
(2.215686274509804, 0.0005172979968281476)
(2.2549019607843137, 0.0010417048249144367)
(2.2941176470588234, 0.0017511617619410998)
(2.3333333333333335, 0.0018022298035003266)
(2.372549019607843, 0.0013781875804013768)
(2.411764705882353, 0.0012117818794052826)
(2.450980392156863, 0.0013730554994830838)
(2.4901960784313726, 0.0015431303408229445)
(2.5294117647058822, 0.0015628898355110766)
(2.568627450980392, 0.001404373745775719)
(2.607843137254902, 0.001175828856855748)
(2.6470588235294117, 0.0010002025866736074)
(2.6862745098039214, 0.0008061593827232016)
(2.7254901960784315, 0.0006048547749173208)
(2.764705882352941, 0.0004503790490231202)
(2.803921568627451, 0.0003800011880675665)
(2.843137254901961, 0.00025806243695638637)
(2.8823529411764706, 8.082239956713267e-5)
(2.9215686274509802, 8.093873166830326e-5)
(2.9607843137254903, 0.00022347141603505424)
(3.0, 0.00039137742326047657)
(3.0392156862745097, 0.0005680392793487885)
(3.0784313725490198, 0.0007095801819917089)
(3.1176470588235294, 0.0007448287358831812)
(3.156862745098039, 0.0006311799161251003)
(3.1960784313725488, 0.00046399220499581686)
(3.235294117647059, 0.00030654263957988426)
(3.2745098039215685, 0.00022108586409358536)
(3.313725490196078, 0.00023746853209224752)
(3.3529411764705883, 0.00024185894921519775)
(3.392156862745098, 0.00021598330510584269)
(3.4313725490196076, 0.00021393756984362748)
(3.4705882352941178, 0.00026916705224417807)
(3.5098039215686274, 0.00029136940338384535)
(3.549019607843137, 0.00029911127730582887)
(3.588235294117647, 0.0003217311346440521)
(3.627450980392157, 0.0003482992529041017)
(3.6666666666666665, 0.00037279770348575697)
(3.7058823529411766, 0.0003835753123727672)
(3.7450980392156863, 0.00038011205589426144)
(3.784313725490196, 0.00035815753223768937)
(3.8235294117647056, 0.0003107810423016698)
(3.8627450980392157, 0.0002724447626175372)
(3.9019607843137254, 0.000252928024500317)
(3.941176470588235, 0.00017510286429641051)
(3.980392156862745, 7.225521471031469e-5)
(4.019607843137255, 0.00016610398519839134)
(4.0588235294117645, 0.00031845036486707125)
(4.098039215686274, 0.00042550689473293187)
(4.137254901960784, 0.0004951890021777779)
(4.176470588235294, 0.0005412685868994444)
(4.215686274509804, 0.0005872448385312433)
(4.254901960784314, 0.0005906439220953165)
(4.294117647058823, 0.0005395820680394468)
(4.333333333333333, 0.0004961053285800898)
(4.372549019607843, 0.0004472914366814003)
(4.411764705882353, 0.0003728911074230489)
(4.450980392156863, 0.00029295707234176175)
(4.490196078431373, 0.00021806336778802842)
(4.529411764705882, 0.0001460946732672039)
(4.568627450980392, 0.0001187874020820094)
(4.607843137254902, 0.00011700064513234866)
(4.647058823529412, 0.00012704643247738373)
(4.686274509803922, 0.00015807213617862406)
(4.7254901960784315, 0.00020335698002517386)
(4.764705882352941, 0.000254248811181768)
(4.803921568627451, 0.000287139156849442)
(4.8431372549019605, 0.0003319950133974766)
(4.88235294117647, 0.00040309572942567954)
(4.921568627450981, 0.0004888159456399855)
(4.96078431372549, 0.0005408681426778909)
(5.0, 0.0005734920121289633)
};
